Time-Space Efficient Regression Testing for Configurable Systems

Configurable systems are those that can be adapted from a set of options. They are prevalent and testing them is important and challenging. Existing approaches for testing configurable systems are either unsound (i.e., they can miss fault-revealing configurations) or do not scale. This paper proposes EvoSPLat, a regression testing technique for configurable systems. EvoSPLat builds on our previously-developed technique, SPLat, which explores all dynamically reachable configurations from a test. EvoSPLat is tuned for two scenarios of use in regression testing: Regression Configuration Selection (RCS) and Regression Test Selection (RTS). EvoSPLat for RCS prunes configurations (not tests) that are not impacted by changes whereas EvoSPLat for RTS prunes tests (not configurations) which are not impacted by changes. Handling both scenarios in the context of evolution is important. Experimental results show that EvoSPLat is promising. We observed a substantial reduction in time (22%) and in the number of configurations (45%) for configurable Java programs. In a case study on a large real-world configurable system (GCC), EvoSPLat reduced 35% of the running time. Comparing EvoSPLat with sampling techniques, 2-wise was the most efficient technique, but it missed two bugs whereas EvoSPLat detected all bugs four times faster than 6-wise, on average.

==> fromsplatpaper.tex <==
%%\newpage
\section{Technique}
\label{sec:technique}

\marcelo{This text is from our SPLat paper  $>>$}
 
Given a test for a configurable system, \SPLKorat{} determines all \relevant{}
configurations on which the test should be run. Each configuration run executes
a unique trace of the test\Space{ (which may produce a unique outcome)}.
\SPLKorat{} executes the test on one configuration, observes the values of 
configuration \options, and uses these values to determine which configurations
can be safely pruned.  \SPLKorat{} repeats this process until it explores all
\relevant{} configurations or until it reaches a specified bound on the number
of configurations. We first describe the feature model interface and then the
core algorithm.

\subsection{Feature Model Interface}

\figref{fmInterface} shows the code snippet that defines the
\CodeIn{FeatureModel} interface\Space{ denoting a feature model}.\Space{ The
\SPLKorat{} algorithm relies on the implementation of this interface.}  The
type \CodeIn{FeatureVar} denotes a feature variable.  A \CodeIn{VarAssign}
object encodes an assignment of boolean values to feature variables.  An
assignment can be \definit{complete}, assigning values to all the features, or
\definit{partial}, assigning values to a subset of the features.  A complete
assignment is \definit{valid} if it satisfies the constraints of the feature
model.  A partial assignment is \definit{satisfiable} if it can be extended to
a valid complete assignment.

%%\begin{figure}[b]
\begin{figure}[h!]
\vspace{2ex}
\normalsize
%\begin{Verbatim}[xleftmargin=10mm,numbers=left,numbersep=6pt,commandchars=\|\[\]]
%\begin{Verbatim}[frame=single]
\begin{lstlisting}[xleftmargin=2pt,framexleftmargin=-1pt,framexrightmargin=-3pt,framexbottommargin=1pt]
class FeatureVar {...}
class VarAssign { ...
 Map<FeatureVar, boolean> map; ...}
interface FeatureModel {
 Set<Assign> getValid(Assign a);
 boolean isSatisfiable(Assign a);
 boolean isMandatory(FeatureVar v);
 boolean getMandatoryValue(FeatureVar v);
}
\end{lstlisting}
%\end{Verbatim}
\normalsize
\caption{Feature Model Interface}
\label{fig:fmInterface}
\end{figure}

The \CodeIn{FeatureModel} interface provides queries for determining the
validity of feature assignments, obtaining valid configurations, and checking
if particular informed features are mandatory. Given an assignment $\alpha$, the
method \CodeIn{getValid()} returns the set of all complete assignments that
(1)~agree with $\alpha$ on the values of feature variables in $\alpha$ and
(2)~assign the values of the remaining feature variables to make the complete assignment valid.
If the set is not empty for $\alpha$, we say that $\alpha$ is
\definit{\satisfiable}; the method \CodeIn{isSatisfiable()} checks this. The
method \CodeIn{isMandatory()} checks if a feature is mandatory according to the
feature model and the method \CodeIn{getMandatoryValue()} returns the mandatory
value for the informed feature.  We build on a SAT solver (SAT4J~\cite{sat4j})
to implement these feature model operations.

\subsection{Main Algorithm}

\figref{splKoratAlgorithm} lists the \SPLKorat{} algorithm.  It takes as input a
test \CodeIn{t} for a configurable system and a feature model \CodeIn{fm}.  To
enable exploration, the algorithm maintains a \CodeIn{state} that stores the
values of feature variables (line~\ref{state}) and a \CodeIn{stack} of feature
variables that are read during the latest test execution (line~\ref{stack}). 
\SPLKorat{} performs a mostly stateless exploration of paths: it does not store,
restore, or compare program states as done in stateful model
checking~\cite{apel-icse2013, damorim-issta2007, kastner-fosd2012,
chpkim-issre12,rhein-jpf2011}; instead, \SPLKorat{} stores only the feature
decisions made along one path and re-executes the code to explore different
program paths, which corresponds to valid and dynamically reachable
configurations.  To that end, \SPLKorat{} needs to be able to set the values of
feature variables, to observe the accesses to feature variables during a test
run, and to re-execute the test from the beginning.

The algorithm first initializes the values of feature variables (lines
\ref{initStart}--\ref{initEnd}) using the feature model interface\Space{
introduced in the previous subsection}.  Mandatory features are set to the only
value they can have, and optional features are initially set to \CodeIn{false}.
Note that initial assignment may be invalid for the given feature model.  For
example, initially setting feature variables to \texttt{false} would violate
the constraint in our Notepad example.  We describe later how \SPLKorat{}
enforces satisfiability \emph{during} execution (in line~\ref{notify1}).  It
adjusts the assignment of values to feature variables \emph{before} test
execution gets to exercise code based on an invalid configuration.  Such
scenario could potentially lead to a ``false alarm'' test failure\Comment{ that
is due to running a test against an invalid configuration} as opposed to
revealing an actual bug in the code under test.  Note that the calls to
\CodeIn{state.put()} both in the initialization block and elsewhere not only
map a feature variable to a boolean value in the state maintained by
\SPLKorat{} but also set the value of the feature variable referred to by the
code under test.

\SPLKorat{} then instruments (line~\ref{instrument}) the code under test to
observe feature variable reads.  Conceptually, for each read of an optional
feature variable (\eg\, reading variable \CodeIn{TOOLBAR} in the code
\CodeIn{if(TOOLBAR)} from \figref{examplespl}), \SPLKorat{} replaces the read
with a call to the \CodeIn{notifyFeatureRead()} method shown in
\figref{splKoratAlgorithm}.  The reads are statically instrumented so that they
can be intercepted just before they happen during test execution.  Mandatory
feature variable reads need not be instrumented because the accessed values
remain constant for all configurations.

%%  (for ease of implementation, our implementation currently instruments all 
%% feature accesses).

\input{main-algo}

\SPLKorat{} next runs the test (line~\ref{runexecution}).  The test execution
calls the method \CodeIn{notify\-Feature\-Read()} whenever it is about to read a
feature variable.\Space{\footnote{More precisely, it is an ``optional feature''
but we simply use ``feature'' because the algorithm need not handle mandatory
features further.}}  When that happens, \SPLKorat{} pushes the feature variable
being read on the \CodeIn{stack} if it is not already there, effectively
recording the order of the first reads of variables.  This \CodeIn{stack}
enables backtracking over the values of read feature variables. An important
step occurs during the call to \CodeIn{notify\-Feature\-Read()}
(line~\ref{notify1}).  The initial value assigned to the reached feature
variable may make the configuration unsatisfiable.  More precisely, at the
beginning of the exploration, \SPLKorat{} sets an optional feature value to
\CodeIn{false}.  When the code is about to read the optional feature,
\SPLKorat{} checks whether the \CodeIn{false} value is consistent with the
feature model, \ie\  whether the \emph{partial} assignment of values to feature
variables on the \CodeIn{stack} is \satisfiable{} for the given feature model. 
If it is, \SPLKorat{} leaves the feature as is.  If not, \SPLKorat{} changes
the feature to \CodeIn{true}.

Note that updating a feature variable to \CodeIn{true} \emph{guarantees} that
the new partial assignment is \satisfiable{}.  The update occurs \emph{before}
execution could have observed the old value which would make the assignment
unsatisfiable. The reason why this change of value keeps the assignment
\satisfiable{} follows from the overall correctness of the \SPLKorat{}
algorithm: it explores only satisfiable partial assignments
(line~\ref{nextValid}), and it checks if the assignment is \satisfiable{} in
\emph{every} variable read (line~\ref{notify1}); thus, if a\Comment{ smaller}
partial assignment was \satisfiable{} considering all features on the
\CodeIn{stack}, then it must be possible to extend that assignment with at
least one value for the new feature that was not on the \CodeIn{stack} but is
being added.  If the variable associated with the new feature stores
\CodeIn{false} at the moment execution accesses that variable, and if the
partial assignment including that feature variable is \emph{not} \satisfiable,
then we can change the value to \CodeIn{true} (line~\ref{notify2}).  Recall
that optional feature variables are initialized to \CodeIn{false}.

After finishing one test execution for one specific configuration, \SPLKorat{}
effectively covers a set of configurations.  This set can be determined by
enumerating every complete assignment that (1)~has the same values as the
partial assignment specified by variables \CodeIn{state} and \CodeIn{stack}
(lines~\ref{partialAssignmentsStart}--\ref{partialAssignments}) and (2)~is
valid according to the feature model (line~\ref{configsExecuted}).

\SPLKorat{} then determines the next configuration to execute by backtracking on
the \CodeIn{stack} (lines \ref{nextStart}--\ref{nextEnd}).  If the last read
feature has value \CodeIn{true}, then \SPLKorat{} has explored both values of
that feature, and it is popped off the stack (lines\ref{nextPop1}--\ref{nextPop2}).  
If the last read feature has value \CodeIn{false}, then \SPLKorat{} has explored
only the \CodeIn{false} value, and the feature should be set to \CodeIn{true}
(lines\ref{nextTrue1}--\ref{nextTrue2}). Another important step occurs now
(line~\ref{nextValid}).  While the backtracking over the\CodeIn{stack} found a
partial assignment to explore, it can be the case that this assignment is not
\satisfiable{} for the feature model. In that case, \SPLKorat{} keeps searching
for the next \satisfiable{} assignment to run.  If no such assignment is found,
the \CodeIn{stack} becomes empty, and \SPLKorat{} terminates.



\subsection{Example Run}


We demonstrate \SPLKorat{} on the example from \figref{examplespl}.
According to the feature model (\figref{featuremodel}),
\CodeIn{NOTEPAD} and \CodeIn{BASE} are the only mandatory features and
are set to \CodeIn{true}\Space{ (both in \CodeIn{state} and in the
program)}.  The other three feature variables are optional and
therefore \SPLKorat{} instruments their reads (\figref{examplespl1},
lines 7, 11, 20, and 23).  Conceptually, the exploration starts
from the configuration $MTW=000$.

When the test begins execution, \CodeIn{notify\-Feature\-Read()} is
first called when \CodeIn{TOOLBAR} is read.  \CodeIn{TOOLBAR} is
pushed on the stack, and because its assignment to \CodeIn{false} is
\satisfiable{} for the feature model, its value remains unchanged
(\ie\ stays \CodeIn{false} as initialized).  Had the feature model
required \CodeIn{TOOLBAR} to be \CodeIn{true}, the feature's value
would have been set to \CodeIn{true} at this point.

With \CodeIn{TOOLBAR} set to \CodeIn{false}, no other feature
variables are read before the test execution finishes. (In particular,
\CodeIn{WORDCOUNT} on line 11 is not read because that line is
not executed when \CodeIn{TOOLBAR} is \CodeIn{false}.)  Therefore,
this one execution covers configurations $MTW=-0-$ where $-$ denotes a
``don't care'' value.  However, configurations $MTW=00-$ are invalid
for the given feature model, so this one execution covers two valid
configurations where \CodeIn{TOOLBAR} is false and \CodeIn{MENUBAR} is true
(\CodeIn{MTW=10-}). Note that even though the value of \CodeIn{WORDCOUNT} does
not matter here, it is given a value nonetheless for an execution because in an
execution, each variable must have a concrete value. So let us say
\CodeIn{MTW=100} here.

\SPLKorat{} next re-executes the test with \CodeIn{TOOLBAR} set to
\CodeIn{true}, as it is satisfiable for the feature model.
\CodeIn{WORDCOUNT} is encountered this time, but it can remain
\CodeIn{false}, and the execution completes, covering \CodeIn{MTW=-10} (again,
for an execution, all variables need to be set, so let us say that
\CodeIn{MTW=010} is what actually executes).
\SPLKorat{} then sets \CodeIn{WORDCOUNT} to
\CodeIn{true}, and the execution completes, covering \CodeIn{MTW=-11} (let us
say \CodeIn{MTW=011} was used). \SPLKorat{} finally pops off \CodeIn{WORDCOUNT}
from the stack because both its values have been explored, and pops
off \CodeIn{TOOLBAR} for the same reason, so the exploration finishes
because the stack is empty\Space{ and there are no other configurations to
explore}. In summary, the test's first execution covers \CodeIn{MTW=10-}
(\CodeIn{MTW=100} is executed), second execution covers \CodeIn{MTW=-10}
(\CodeIn{MTW=010} is executed) and third execution covers \CodeIn{MTW=-11}
(\CodeIn{MTW=011} is executed). Therefore, the technique covers all 6 valid
configurations by executing just three configurations.

\subsection{Reset Function}
\label{sec:resetFunction}

While a stateless exploration technique such as \SPLKorat{} does not need to
store and restore program state in the middle of execution like a stateful
exploration technique does, the stateless exploration does need to be able to
restart a new execution from the initial program state unaffected by the
previous execution.\Space{ Put another way, every execution of the program
needs to start with the same program state.}  Restarting an execution with a
new runtime (\eg\ spawning a new \definit{Java Virtual Machine (JVM)} in Java)
is the simplest solution, but it can be both inefficient and unsound.  It is
inefficient because even without restarting the runtime, the different
executions may be able to share a runtime and still have identical initial
program states, \eg\  if the test does not update any static variables in the
JVM state.  It can be unsound because a new runtime may not reset the program
state changes made by the previous executions (\eg\ previous executions having
sent messages to other computers or having performed I/O operations such as
database updates).  We address\Space{ both of} these issues by sharing the
runtime between executions and requiring the user to provide a \definit{reset
function} that can be called at the beginning of the test.

Our sharing of the runtime between executions means that settings that would
normally be reset automatically by creating a new runtime must now be manually
reset.  For example, Java static initializers must now be called from the reset
function because classes are loaded only once.  However, we believe that the
benefit of saving time by reusing the runtime outweighs the cost of this
effort, which could be alleviated by a program analysis tool.  Moreover, for
the Groupon code used in our evaluation, the testing infrastructure was already
using the reset function (developed independently and years before this
research); between any test execution, the state (of both memory and database)
is reset (by rolling back the database transaction from the previous test and
overwriting the state changes in the \CodeIn{tearDown} and/or \CodeIn{setUp}
blocks after/before each test).

\subsection{Potential Optimization\Space{ for Interfacing with the Feature Model}}
\label{sec:featureModelOptimization}

The algorithm in \figref{splKoratAlgorithm} is not optimized in how it
interfaces with the feature model.  The feature model is treated as a blackbox,
read-only artifact that is oblivious to the exploration state consisting of the
\CodeIn{state} and \CodeIn{stack}. Consequently, the
\CodeIn{\Space{Feature\-Model.}is\-Satisfiable()} and
\CodeIn{\Space{Feature\-Model.\-}getValid()} methods are executed as if the
exploration state was completely new every time, even if it just incrementally
differs from the previous exploration state.  For example, when running the
test from \figref{examplespl}, \SPLKorat{} asks the feature model if
$MTW=-1-$\Comment{ (\CodeIn{TOOLBAR=true})} is satisfiable (line~\ref{nextValid}
of the \SPLKorat{} algorithm) after the assignment $MTW=-0-$.  The feature
model replies \CodeIn{true} as it can find a configuration with the feature
\CodeIn{TOOLBAR} set to true.  Then when \CodeIn{WORDCOUNT} is encountered
while \CodeIn{TOOLBAR=true}, \SPLKorat{} asks the feature model if the
assignment $MTW=-10$ (\CodeIn{TOOLBAR=true} \textit{and}
\CodeIn{WORDCOUNT=false}) is satisfiable (line~\ref{notify1} of the \SPLKorat{}
algorithm)\Space{, although \CodeIn{TOOLBAR} is already known to be
\CodeIn{true}}.  Note that the feature model is not aware of the similarity
between the consecutive calls for $MTW=-1-$ and $MTW=-10$.  But if it were, it
would only have to check the satisfiability of \CodeIn{WORDCOUNT=false}.

The change to the algorithm to enable this synchronization between the
exploration state and the feature model is simple: every time a feature
variable is pushed on the \CodeIn{stack}, constrain the feature model with the
feature's value, and every time a feature variable is popped off the
\CodeIn{stack}, remove the corresponding feature assignment from the feature
model.  A feature model that can be updated implies that it should support
incremental solving, \ie\ a feature model should not have to always be solved
in its entirety. Our current \SPLKorat{} tool for Java does not exploit
incremental solving, meaning that the tool has not reached the limits of the
underlying technique and can be made even faster.

%We did not implement a
%feature model with incremental solving because the SPL subjects we
%evaluated for Java do not have a very large number of configurations,
%and the time spent in the calls to the feature model turned out to be
%negligible compared to the rest of the test execution.

\subsection{Implementation}

We implemented two versions of \SPLKorat{}, one for Java and one for Ruby on
Rails.  We selected these two languages motivated by the subject programs used
in our experiments (Section~\ref{sec:evaluation}).

For Java, we implemented \SPLKorat{} on top of the publicly available
\texttt{Korat} solver for imperative predicates~\cite{KoratWebPage}. Korat
already provides code instrumentation (based on the BCEL library for Java
bytecode manipulation) to monitor field accesses, and provides basic
backtracking over the accessed fields.  The feature variables in our Java
subjects were already represented as fields. The main extension for \SPLKorat{}
was to integrate Korat with a SAT solver for checking satisfiability of partial
assignments with respect to feature models.  As mentioned earlier, we used
SAT4J~\cite{sat4j}.

For Ruby on Rails, we have an even simpler implementation that only monitors
accesses to feature variables.  We did not integrate  a SAT solver, because the
subject code did not have a formal feature model and thus we treated all
combinations of feature variables as valid.

\marcelo{$<<$ Text from SPLat paper ends here.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Stackless Technique}
%\label{sec:stacklessTechnique}

%Record feature accesses and try on all combinations. 

\marcelo{Darko, this was commented in the text of SPLat paper.
  Sabrina, pointed out.$>>$}

\subsection{Regression Testing}
\label{sec:regressionTesting}

Automated tests are typically written to be used in regression testing, where
they are run not only once but multiple times on evolving versions of the code
under test.  An important question is how to further speed up \SPLKorat for
regression testing.  When we run a test for the first time, we can record which
configurations were \relevant [or whatever term you use] for this test.  We can
compactly encode all these configurations as a decision tree for each test. 
For example, \CodeIn{if (A) \{ if (B) ... \} ...} would have a tree like this:

\begin{verbatim}
       A
  true/ \false
      B  .
 true/ \false
\end{verbatim}
   
Moreover, a number of tests can share these trees.  [For Sarfraz: you have an
INS here, so we can repeat the entire INS/TestEra/Korat 12 years after! :)]
Then, when the code under test (or the test code itself) is changed, we need
not run the full \SPLKorat but can reuse the configuration tree from the
previous run and execute only those configurations.  [For Peter: note that this
should be added on the to-do list for the experiments anyhow: to get the more
precise overhead of \SPLKorat, you'd want to run (1) \SPLKorat as now and (2)
only the \relevant configurations on JVMReset, and then compare the times;
comparing what you do now time reduction vs. configuration number reduction is
imprecise (although probably quite accurate!) because different configurations
can be taking different time (although they are probably quite similar).]

However, note that there is a challenge here that the change (in the code under
test or the test itself) could have invalidated the set of \relevant
configurations.  More precisely, there can be (1) configurations that are not
 encoded in the tree but became \relevant after the change, and/or (2)
configurations that are encoded in the tree but are not \relevant any more
after the change.  We present an algorithm, called \RegressionSPLKorat that can
take an old tree, execute it on the new code, and do the following:
\begin{enumerate}
\item If the tree remained a precise encoding of all the \relevant
configurations, then \RegressionSPLKorat finishes faster than \SPLKorat [let's
h ope we have here 20-30-40-50\% across various tests/programs].
\item If the tree is not precise any more, then \RegressionSPLKorat can
determine that change is required (\ie\  new configurations should be added
and/or some existing configurations should be removed) and can build a new
tree, while running only a bit slower than \SPLKorat [let's hope we have here
only 10\% slowdown].
\end{enumerate}
Since the case where the tree remains the same is much more common in the
 evolution of real code, the speedup gain from case 1 significantly outweighs
the slowdown loss from case 2.

The algorithm \RegressionSPLKorat proceeds as follows. [I have no clue how
exactly it should work :), but the idea is that you don't need to invoke the
solver at all and can only minimally instrument the accesses to feature
variables to check that the variables accessed in the current exploration
actually match what is in the tree from the previous exploration; if you find
any deviation, you can invoke \SPLKorat to run from scratch, or even better
could do something incrementally to only run \SPLKorat on the subtrees where
\RegressionSPLKorat found some change.]

Darko ran across ``Combinatorial Interaction Regression Testing'' while writing
future work: http://cse.unl.edu/~myra/papers/quICSM.pdf



==> gcc_old.tex <==
\section{Configurable System: GCC}
\label{sec:gcc}

We next considered the GNU Compiler Collection (\gcc)~\citep{gcc}, a
large system with hundreds of configuration options~\citep{gccoptions}.

The \gcc{} testing infrastructure runs each test for one specific
configuration, obtained by overriding default option values with
specific options defined in the test.  In contrast, \splat{} runs each test for multiple configurations, fixing
user-defined options and varying the rest of reachable options (/variables), which otherwise would assume default values.  This
approach effectively exercises all reachable configurations up to a
speficied bound on the number of configurations.

%%  and then we applied \tname{} to
%% rank both the failing tests and configurations, as we did in
%% Section~\ref{sec:eval}.  Our primary goal was to see how \tname{}
%% could scale to such a large system and what kind of failures it could
%% find. With the recent work on testing
%% \gcc~\cite{yang-etal-pldi-2011,chen-etal-pldi-2013,le-etal-pldi-2014},
%% we did not expect to find new bugs, but \tname{} did.  As we do not
%% have extensive \gcc{} knowledge to properly classify general
%% failures\Comment{replace ``configurations'' by ``failures''}, we
%% focused our inspection of failures on crashes\Comment{ and incorrect
%%   execution output?}, which provide a stronger indication of a real
%% bug in code. We first give a high-level summary of setup and results,
%% and then more details of applying \tname{} on GCC.

\subsection{Setup}

To deal 
with the high cost of test execution, we focused on a selection of test suites, 
ran \splat{} using a limited number of options, and limited the number of configurations 
per test. \marcelo{I pulled this out as it was referring to non-testing stuff as well as testing stuff. check if makes sense. \Fix{OK}}

\subsubsection{Tests}
Test execution in \gcc{} is time consuming. Considering one configuration per 
test and our running environment, it takes roughly 2s per test run.  We focused on the \CodeIn{gcc-dg} test suite, which contains 3343 tests, as we observed 
from bug-reports a higher incidence of bugs revealed with this suite. 
\Fix{From these 3343 tests, we considered only tests that do not reach a specified bound (100 configurations) so to construct the entire decision tree; otherwise, we can bias the search to a narrow space of configurations, in total 892 tests.}
%\marcelo{why?  is that the bound?  if so, say it explicitly.}
%\marcelo{also, it is important to say that we considered only cases that do not reach a specified bound so to construct the entire decision tree; otherwise, we could bias the search to a narrow space of configurations.}, 
%we used the model from~\cite{sabrina-etal-splc15} to validate the configurations\marcelo{should we care about this?  from i remember splif did not use this and was able to find crashes.  if this is not critical, i suggest to remove it.}. 

\subsubsection{Options}
To make the runtime reasonable, we restricted the number of options that \splat{}
considers (see~\citep{gccoptions}). We used the most 33 frequently cited options in the 
\gcc{} bug reports (from the week of daily versions). 
%The rationale was that more 
%bugs could be found close to where some bugs have been recently reported (we noticed 
%that the top options do not change much across months).

\subsubsection{Versions and Changes}
%We used 8\marcelo{this is super confusing!  at one point you say 8 then 7 combinations are shown.  i understand why is 7 and 8, but it is confusing to the reader anyways.} daily versions\marcelo{You are also using ``daily build'' in the next table (figure 10) which is super confusing} from a week. \marcelo{Sabrina, it is OK to use daily build as every knows it, but use consistently.  I suggest to use +1, +2, and refer to it as evolution (e.g., the evolution +1) and here explain what this means.}  \marcelo{i understand the goal here is not to edit the paper, but it is not a good idea to accumulate poorly edited text.}

%Each version has about 19K functions in \gcc{} core and C/C++ packages.\marcelo{Why this is important?  and What is the definition of a version as in ``Each version''?  I presume the 1-31 functions do not contain this much code. Let alone ``has about 19K'' is way to vague.}

We considerd 7 evolution cycles and 8 daily builds.  We use the symbol
+1 to indicate the evolution from a base date (\Fix{indicate exact
  date}) to the next day.\Fix{use Evolution instead of ``Daily Build''
  in tables to refere to +1, +2, etc.  This symbol associates a pair
  of dates so is an indication of evolution, not a build (a point in
  time).}  We measure the impact of the changed code at function
granularity. The Figure~\ref{tab:changes} shows the amount of
functions that change across daily builds.

\setlength{\tabcolsep}{2.5pt}
\begin{figure}[h!] %was t!
\footnotesize
\centering
\begin{tabular}{|c|c|}
\hline
\emph{Daily Build} & \#~\emph{Functions} \\ \hline
+1 & 31 \\ \hline
+2 & 4  \\ \hline
+3 & 4  \\ \hline
+4 & 15 \\ \hline
+5 & 13 \\ \hline
+6 & 1  \\ \hline
+7 & 8  \\ \hline
\end{tabular}
%\vspace{-2ex}
\caption{\label{tab:changes}The number of functions that change across versions.\Comment{\Fix{NEW}\marcelo{use +1, +2 as I mentioned before. Be consistent!}}}
\end{figure}
\normalsize


\subsection{\tname{} for Configurable Systems}

%\Fix{need to think more how to present this.  as of now it is a bit weird this adaptation for configurable systems}
%
%We describe below the adaptation of \tname{} for handling configurable
%systems, which take configuration options on input.
%
%\begin{itemize}
%\item For each execution $i$ of \tname{} on version $n$, collect two
%  traces: one trace of function calls $\mathit{tfc}_i$ and one trace
%  of variable accesses $\mathit{tv}_i$;
%\item Provided the set $C$ of function changes, obtained from the
%  evolution of version $n$ to version $n+1$, proceed as follows:
%  \begin{itemize}
%    \item Select all traces of variables $\mathit{tv}_i$ for which
%      $\mathit{tfc}_i$ contains some changed function in $C$;
%    \item Partition the set of traces $\mathit{tv}_i$ according to
%      their ``longest common prefix''~--~all traces in the same
%      partition have the same prefix.  For that, sort the traces
%      lexicografically, hierarchical cluster~\Fix{cite} the set of
%      strings from $\mathit{tv}_i$ based on their prefixes\footnote{A
%        40-line Python script for this step is publicly available
%        \url{...}.}, and select the clustering from the hierarchy that
%      maximizes both the number of reported clusters and the number of
%      elements inside each cluster.
%    \item Re-execute \splat{} for each prefix that labels each cluster
%      found in the previous step.  The prefix determines a partial
%      configuration to execute SPLat.
%  \end{itemize}
%\end{itemize}
%
%\subsubsection{Example}
%
%\Fix{...}

\subsubsection{Characterization of function call traces} \Fix{Moved from Setup to here}
%\marcelo{I don't think this is setup.  It looks more part of the methodology.  I suggest you to move this to Section B, if you don't have a better place.}
\Fix{We collected the traces of function calls for each test after \splat{} execution, 
resulting on one trace per configuration. Figure~\ref{fig:pfap} shows the distribution of 
functions covered per test: in the first column there is a boxplot with the distribution on 
number of functions common (COMMNON) to all traces, per test; and, in the second column, a boxplot with 
the distribution on the number of different functions (DIFF) per test. We can observe that there is a lower number of different  
functions compared to the number of common functions.}

\setlength{\tabcolsep}{2.5pt}
\begin{figure}[h!] %was t!
\footnotesize
%\scriptsize
\centering
\begin{tabular}{|c|c|}
\hline
\emph{PFAP} & \#\emph{NumTests}  \\
\hline
[\z0-10[ & 0 \\ \hline
[10-20[ & 0 \\ \hline
[20-30[ & 0 \\ \hline
[30-40[ & 0 \\ \hline
[40-50[ & 0 \\ \hline
[50-60[ & 1 \\ \hline
[60-70[ & 1 \\ \hline
[70-80[ & 72 \\ \hline
[80-90[ & 183 \\ \hline
[90-100] & 33 \\ \hline
\#\emph{Total} & 290 \\ \hline
\end{tabular}
%\vspace{-2ex}
\caption{\label{tab:gcc-caracteristics}Percentage of common function across configuration for each test . FunctionsAlwaysPresent(PFAP). \Fix{NEW}}
\end{figure}
\normalsize

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{plots/pfap.pdf}
\vspace{-2ex}
\caption{The distribution of functions covered per test: COMMON (the number of common functions per test),
 and DIFF (the number of different functions per test). \Fix{We are using 290 tests for while.} \marcelo{Sabrina, I don't understand: is COMMON and DIFF complementary?  If so, I don't understand why you want to show both.  The statistics that I care are: (distribution of) percentage of common function across configuration for each test and (distribution of) percentage of common function across configurations for all tests.}}
%Percentage of Functions that are Always Present (PFAP) per test. \marcelo{This scatterplot is not clear sabrina.  You said, there were only 90 tests and here the y-axis  (*for numtests*) goes from 0-100.  According to that, only one triangle alone is associated to 90+ tests.  My suggestion is to show two boxplots: one to show the distribution of distinct functions covered in each tests and another to show the distribution of FPAPs across all tests.}}
\label{fig:pfap}
\end{figure}

%shows that all considered tests have a high percentage of functions that are always present in its traces.
%\Fix{And we realized that there is a great amount of functions that are always present in all traces of each test. }\marcelo{General: discuss results after you present them.  There is no point in anticipation.}

\subsubsection{Basic RTS}
This experiment measures the number of tests affected by the changes from one 
version to the next one. The insight of \emph{Basic RTS} is to collected all the functions 
that all the tests/configurations depend on, and then select to re-run the entire test for 
the next version, with all its configurations, if any of the functions change.   \marcelo{...}For example,... \Fix{I will provide an example...}

\setlength{\tabcolsep}{2.5pt}
\begin{figure}[h!] %was t!
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|} \hline
\multirow{2}{*}{\emph{Daily Build}} & \emph{Baseline} & \multicolumn{2}{c|}{\emph{Basic RTS}} \\
\cline{2-4}
& Time(h) & Tests Exec.(\%) & Time(h) \\ \hline
+1 & 10.15 & 100 & 10.15 \\ \hline
+2 & 10.15 & 100 & 10.15 \\ \hline
+3 & 10.15 & 0 & 0.0 \\ \hline
+4 & 10.15 & 7.6 & 0.78 \\ \hline
+5 & 10.15 & 100 & 10.15 \\ \hline
+6 & 10.15 & 47 & 5.1 \\ \hline
+7 & 10.15 & 100 & 10.15 \\ \hline
AVG & 10.15 & 65 & 6.64 \\ \hline
\end{tabular}
\caption{\label{tab:basic-rts}Basic RTS. \Fix{We are using 290 tests for while.}
\marcelo{I am **super** suprised that for some evolutions (5 exactly) you could not 
find a mix of cases where some tests run all configurations and some tests run none. 
 For example, on evolution +2 you are saying that all 90 tests had at least one function 
 in the set of modified function across the evolution and I see from Fig. 8 there are only 
 4 changed functions in +2.  This is a very small fraction of a big universe.  So, it 
 is weird for me.  You should be very careful with that Sabrina.} 
 %\Fix{I am being careful, Marcelo. I am confident that the results are correct. To remaind you, we discussed this in our email to Darko a week ago: This happens because there is a small change in the set of functions called through different configurations for a given test (see Figure~\ref{tab:changes}). For example, the test t1 calls 4129 functions through 192 configurations. From those 4129 functions, 3842 are always called (see Figure~\ref{fig:pfap}). This pattern repeats for all tests that I evaluated. Moreover, the set of changed functions in each evolution is relatively low. When a changed function appears on the trace, it appears between the functions that are always called.}
 \Fix{This happens because 67.3\% of the functions appears in all traces of all tests. I 
 checked those functions in the code and I realized that all these functions are always called 
 because when we run a test in GCC, it makes a build of the test before executing it. -->So, 
 these common functions refer to the build of the test.<-- Therefore, whenever a changed function 
 belongs to these common functions, all traces of all tests will be affected, and all tests 
 must be re-executed using Basic RTS approach. But, now that we know why that happens, I believe 
 that it is not necessary to select all tests in this case... maybe one test or one trace of each test 
 must be selected to test this kind of change, do you agree?}\marcelo{Sabrina, you need to be more specific; I don't understand.  If you are sure about it and want to convince me: explain with an example. }
 }
\end{figure}
\normalsize

Figure~\ref{tab:basic-rts} reports \Comment{\marcelo{use illustrate to present/illustrate an idea or example.  here, use ``shows''}}the results for \emph{Basic RTS}. Column 
\emph{Daily Build} represents the daily versions, where we run \splat{} (our baseline) for 
the first version, and collectd the execution time for all tests/configurations in column 
\emph{Baseline: Time(h)}. Next, we calculate the percentage of tests affected by changes from 
the first version and the next one in column \emph{Basic RTS: Tests Exec.(\%)}, i.e., 
the percentage of tests to be re-executed in the next version. Then, we re-run \splat{} 
for the next version with the affected tests, and collect its execution time in column 
\emph{Basic RTS: Time(h)}



%\subsubsection{Non-Basic RTS}
%\Fix{TODO}

%\subsection{Evaluation}



%
%\Fix{...describe the setup: which versions used, ammount of changes...}
%
%\Fix{techniques to compare: SPLat vs. EvoSPLat.  metrics: (1) reduction in number of configurations and time, (2) failures observed}


==> main-algo.tex <==
\begin{figure}[h!]
\vspace{4ex} %% otherwise will print outside margins
\normalsize
%\begin{Verbatim}[xleftmargin=10mm,numbers=left,numbersep=6pt,commandchars=\|\[\]]
\begin{lstlisting}[numbers=left,escapeinside={@}{@},xleftmargin=3.0ex,showstringspaces=false,showtabs=false,xleftmargin=17pt,framexleftmargin=17pt,framexrightmargin=-1pt,framexbottommargin=4pt,numberstyle=\scriptsize]
Stack<FeatureVar> stack;            @\label{stack}@
Map<FeatureVar, Boolean> state;     @\label{state}@

// input, shared with instrumented code
FeatureModel fm; 

void SPLat(Test t) {
 // Initialize features                 @\label{initStart}@
 state = new Map();
 for (FeatureVar f: fm.getFeatureVariables())
  state.put(f, fm.isMandatory(f) ?
               fm.getMandatoryValue(f) : 
               false); @\label{initEnd}@

  // Instrument the code under test
  instrumentOptionalFeatureAccesses();   @\label{instrument}@
  
  do { 

   // Repeatedly run the test
   stack = new Stack();
   t.runInstrumentedTest();             @\label{runexecution}@
   VarAssign pa =                       @\label{partialAssignmentsStart}@
    getPartialAssignment(state, stack); @\label{partialAssignments}@
   print("configs covered: ");
   print(fm.getValid(pa));             @\label{configsExecuted}@

   while (!stack.isEmpty()) {          @\label{nextStart}@
    FeatureVar f = stack.top();
    if (state.get(f)) {                @\label{nextPop1}@
     state.put(f, false); // Restore
     stack.pop();
    } else {                           @\label{nextPop2}\label{nextTrue1}@
     state.put(f, true);
     pa = getPartialAssignment(state, stack);
     if (fm.isSatisfiable(pa)) @\label{nextValid}@
      break;
    }                                  @\label{nextTrue2}@
   }                                   @\label{nextEnd}@

  } while (!stack.isEmpty());
}

// called-back from test execution
void notifyFeatureRead(FeatureVar f) {
 if (!stack.contains(f)) {
  stack.push(f);
  VarAssign pa = 
   getPartialAssignment(state, stack);
  if (!fm.isSatisfiable(pa))          @\label{notify1}@
   state.put(f, true);                @\label{notify2}@
 }
}
\end{lstlisting}
%\end{Verbatim}
\normalsize
\caption{\SPLKoratName{} Algorithm}
\label{fig:splKoratAlgorithm}
%\vspace{-4ex}
\end{figure}


==> resultsTable.tex <==
\setlength{\tabcolsep}{2.5pt}
\def\arraystretch{0.9}%
\begin{figure*}[h!]
\centering
\scriptsize
%\tiny
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% first row

%%%%%%%%%%%%%%%%%% companies
  \begin{tabular}{|c|r|r|r|} \hline
    test & \CodeIn{SPLat} & \tname{} & Red(\%)\\ \hline
    \multicolumn{3}{c}{\textbf{101Companies [All]}} \\ \hline
$t_{1}$ & 24 & 22.03 & 8.21 \\ \hline 
$t_{2}$ & 96 & 72.09 & 24.91 \\ \hline 
$t_{3}$ & 18 & 10.8 & 40.0 \\ \hline 
$t_{4}$ & 72 & 41.91 & 41.79 \\ \hline 
$t_{5}$ & 96 & 71.62 & 25.4 \\ \hline 
$t_{6}$ & 96 & 68.79 & 28.34 \\ \hline 
$t_{7}$ & 24 & 23.37 & 2.62 \\ \hline 
$t_{8}$ & 24 & 23.44 & 2.33 \\ \hline 
$t_{9}$ & 24 & 23.52 & 2.0 \\ \hline 
$t_{10}$ & 24 & 22.51 & 6.21 \\ \hline 
$t_{11}$ & 96 & 64.65 & 32.66 \\ \hline 
$t_{12}$ & 24 & 17.11 & 28.71 \\ \hline 
$t_{13}$ & 96 & 63.97 & 33.36 \\ \hline 
$t_{14}$ & 14 & 7.34 & 47.57 \\ \hline 
$t_{15}$ & 49 & 24.9 & 49.18 \\ \hline 
$t_{16}$ & 97 & 66.57 & 31.37 \\ \hline 
$t_{17}$ & 8 & 6.77 & 15.38 \\ \hline 
$t_{18}$ & 2 & 2.0 & 0.0 \\ \hline 
$t_{19}$ & 4 & 3.29 & 17.75 \\ \hline 
$t_{20}$ & 4 & 4.0 & 0.0 \\ \hline 
$t_{21}$ & 4 & 4.0 & 0.0 \\ \hline 
$t_{22}$ & 4 & 4.0 & 0.0 \\ \hline 
\textbf{AVG} & - & - & 19.9\\\hline

%\end{tabular}

%% %%%%%%%%%%%%%%%%%% gpl
%\begin{tabular}{|c|r|r|} \hline
%    test & \CodeIn{SPLat} & \tname{} \\ \hline
    \multicolumn{3}{c}{\textbf{GPL[All]}} \\ \hline
$t_1$ & 19 & 17.00 & 10.53 \\ \hline 
$t_2$ & 49 & 49.00 & 0.0 \\ \hline 
$t_3$ & 7 & 7.00 & 0.0 \\ \hline 
$t_4$ & 42 & 41.13 & 2.07 \\ \hline 
$t_5$ & 6 & 4.00 & 33.33 \\ \hline 
$t_6$ & 5 & 5.00 & 0.0 \\ \hline 
$t_7$ & 7 & 4.00 & 42.86 \\ \hline 
$t_8$ & 49 & 49.00 & 0.0 \\ \hline 
$t_9$ & 49 & 24.70 & 49.59 \\ \hline 
$t_{10}$ & 10 & 5.00 & 50.0 \\ \hline 
$t_{11}$ & 7 & 3.91 & 44.14 \\ \hline 
$t_{12}$ & 7 & 3.91 & 44.14 \\ \hline 
$t_{13}$ & 5 & 2.32 & 53.6 \\ \hline 
$t_{14}$ & 7 & 5.00 & 28.57 \\ \hline 
$t_{15}$ & 7 & 7.00 & 0.0 \\ \hline 
$t_{16}$ & 5 & 4.33 & 13.4 \\ \hline 
$t_{17}$ & 5 & 5.00 & 0.0 \\ \hline 
$t_{18}$ & 10 & 5.00 & 50.0 \\ \hline 
$t_{19}$ & 40 & 18.00 & 55.0 \\ \hline 
$t_{20}$ & 50 & 23.93 & 52.14 \\ \hline 
$t_{21}$ & 62 & 35.35 & 42.98 \\ \hline 
$t_{22}$ & 8 & 2.77 & 65.38 \\ \hline 
$t_{23}$ & 5 & 4.20 & 16.0 \\ \hline 
$t_{24}$ & 49 & 49.00 & 0.0 \\ \hline 
$t_{25}$ & 5 & 4.33 & 13.4 \\ \hline 
\textbf{AVG} & - & - & 26.69\\\hline
\end{tabular}


\begin{tabular}{|c|r|r|r|} \hline
    test & \CodeIn{SPLat} & \tname{}  & Red(\%)\\ \hline
    \multicolumn{3}{c}{\textbf{DesktopSearcher [All]}} \\ \hline
$t_{1}$ & 26 & 15.38 & 40.85 \\ \hline 
$t_{2}$ & 26 & 15.38 & 40.85 \\ \hline 
$t_{3}$ & 26 & 15.38 & 40.85 \\ \hline 
$t_{4}$ & 26 & 15.38 & 40.85 \\ \hline 
$t_{5}$ & 26 & 15.41 & 40.73 \\ \hline 
$t_{6}$ & 31 & 17.36 & 44.0 \\ \hline 
$t_{7}$ & 28 & 15.71 & 43.89 \\ \hline 
$t_{8}$ & 32 & 17.98 & 43.81 \\ \hline 
$t_{9}$ & 26 & 13.63 & 47.58 \\ \hline 
$t_{10}$ & 26 & 13.61 & 47.65 \\ \hline 
$t_{11}$ & 26 & 15.41 & 40.73 \\ \hline 
$t_{12}$ & 20 & 11.7 & 41.5 \\ \hline 
$t_{13}$ & 40 & 23.29 & 41.78 \\ \hline 
$t_{14}$ & 31 & 17.7 & 42.9 \\ \hline 
$t_{15}$ & 26 & 15.41 & 40.73 \\ \hline 
$t_{16}$ & 26 & 15.41 & 40.73 \\ \hline 
$t_{17}$ & 26 & 15.41 & 40.73 \\ \hline 
$t_{18}$ & 26 & 15.41 & 40.73 \\ \hline 
$t_{19}$ & 16 & 14.91 & 6.81 \\ \hline 
$t_{20}$ & 16 & 10.49 & 34.44 \\ \hline 
$t_{21}$ & 8 & 5.48 & 31.5 \\ \hline 
$t_{22}$ & 2 & 1.25 & 37.5 \\ \hline 
$t_{23}$ & 8 & 5.48 & 31.5 \\ \hline 
$t_{24}$ & 8 & 5.48 & 31.5 \\ \hline 
$t_{25}$ & 8 & 5.48 & 31.5 \\ \hline 
$t_{26}$ & 2 & 1.17 & 41.5 \\ \hline 
$t_{27}$ & 8 & 6.03 & 24.62 \\ \hline 
$t_{28}$ & 8 & 6.03 & 24.62 \\ \hline 
$t_{29}$ & 8 & 6.0 & 25.0 \\ \hline 
$t_{30}$ & 8 & 6.0 & 25.0 \\ \hline 
$t_{31}$ & 2 & 1.33 & 33.5 \\ \hline 
$t_{32}$ & 8 & 5.48 & 31.5 \\ \hline 
$t_{33}$ & 8 & 4.61 & 42.37 \\ \hline 
$t_{34}$ & 8 & 4.39 & 45.13 \\ \hline 
$t_{35}$ & 8 & 4.39 & 45.13 \\ \hline 
$t_{36}$ & 13 & 7.09 & 45.46 \\ \hline 
$t_{37}$ & 13 & 7.35 & 43.46 \\ \hline 
$t_{38}$ & 13 & 7.35 & 43.46 \\ \hline 
$t_{39}$ & 13 & 7.35 & 43.46 \\ \hline 
$t_{40}$ & 13 & 7.35 & 43.46 \\ \hline 
$t_{41}$ & 14 & 7.67 & 45.21 \\ \hline 
$t_{42}$ & 22 & 12.86 & 41.55 \\ \hline 
$t_{43}$ & 9 & 7.02 & 22.0 \\ \hline 
$t_{44}$ & 22 & 12.86 & 41.55 \\ \hline 
\textbf{AVG} & - & - & 38.04\\\hline


% %%%%%%%%%%%%%%%%% minepump
%\begin{tabular}{|c|r|r|} \hline
%    test & \CodeIn{SPLat} & \tname{} \\ \hline
    \multicolumn{3}{c}{\textbf{MinePump[All]}} \\ \hline
$t_1$ & 9 & 6.43 & 28.56 \\ \hline 
$t_2$ & 24 & 18.03 & 24.87 \\ \hline 
$t_3$ & 48 & 33.23 & 30.77 \\ \hline 
\textbf{AVG} & - & - & 28.07\\\hline
%\end{tabular}

\end{tabular}


%% %%%%%%%%%%%%%%%%%% notepad
\begin{tabular}{|c|r|r|r|} \hline
    test & \CodeIn{SPLat} & \tname{}  & Red(\%)\\ \hline
    \multicolumn{3}{c}{\textbf{Notepad [100]}} \\ \hline
$t_1$ & 100 & 75.22 & 24.78 \\ \hline 
$t_2$ & 100 & 74.63 & 25.37 \\ \hline 
$t_3$ & 100 & 74.05 & 25.95 \\ \hline 
$t_4$ & 100 & 73.49 & 26.51 \\ \hline 
$t_5$ & 100 & 75.67 & 24.33 \\ \hline 
$t_6$ & 100 & 75.29 & 24.71 \\ \hline 
$t_7$ & 100 & 74.63 & 25.37 \\ \hline 
$t_8$ & 100 & 75.22 & 24.78 \\ \hline 
$t_9$ & 100 & 74.63 & 25.37 \\ \hline 
$t_{10}$ & 100 & 74.63 & 25.37 \\ \hline 
$t_{11}$ & 100 & 75.22 & 24.78 \\ \hline 
$t_{12}$ & 96 & 71.78 & 25.23 \\ \hline 
$t_{13}$ & 96 & 73.35 & 23.59 \\ \hline 
$t_{14}$ & 96 & 73.05 & 23.91 \\ \hline 
$t_{15}$ & 96 & 73.05 & 23.91 \\ \hline 
$t_{16}$ & 96 & 73.05 & 23.91 \\ \hline 
$t_{17}$ & 96 & 73.05 & 23.91 \\ \hline 
$t_{18}$ & 96 & 73.05 & 23.91 \\ \hline 
$t_{19}$ & 96 & 72.75 & 24.22 \\ \hline 
$t_{20}$ & 96 & 71.78 & 25.23 \\ \hline 
$t_{21}$ & 96 & 69.55 & 27.55 \\ \hline 
$t_{22}$ & 96 & 70.44 & 26.63 \\ \hline 
$t_{23}$ & 96 & 70.44 & 26.63 \\ \hline 
$t_{24}$ & 96 & 72.10 & 24.9 \\ \hline 
$t_{25}$ & 96 & 72.10 & 24.9 \\ \hline 
$t_{26}$ & 96 & 71.79 & 25.22 \\ \hline 
$t_{27}$ & 96 & 68.27 & 28.89 \\ \hline 
$t_{28}$ & 100 & 72.29 & 27.71 \\ \hline 
$t_{29}$ & 100 & 72.29 & 27.71 \\ \hline 
$t_{30}$ & 100 & 73.22 & 26.78 \\ \hline 
$t_{31}$ & 100 & 72.29 & 27.71 \\ \hline 
$t_{32}$ & 100 & 75.29 & 24.71 \\ \hline 
$t_{33}$ & 100 & 69.83 & 30.17 \\ \hline 
$t_{34}$ & 100 & 76.46 & 23.54 \\ \hline 
$t_{35}$ & 100 & 75.44 & 24.56 \\ \hline 
$t_{36}$ & 100 & 76.62 & 23.38 \\ \hline 
$t_{37}$ & 100 & 73.63 & 26.37 \\ \hline 
$t_{38}$ & 100 & 75.76 & 24.24 \\ \hline 
$t_{39}$ & 100 & 75.76 & 24.24 \\ \hline 
$t_{40}$ & 100 & 75.76 & 24.24 \\ \hline 
$t_{41}$ & 100 & 75.76 & 24.24 \\ \hline 
$t_{42}$ & 100 & 75.76 & 24.24 \\ \hline 
$t_{43}$ & 100 & 75.76 & 24.24 \\ \hline 
\textbf{AVG} & - & - & 25.3\\\hline
%\end{tabular}

%%%%%%%%%%%%%%%%%% xstream
%\begin{tabular}{|c|r|r|} \hline
%    test & \CodeIn{SPLat} & \tname{} \\ \hline
    \multicolumn{3}{c}{\textbf{XStream [All]}} \\ \hline
$t_1$ & 2 & 1.89 & 5.5 \\ \hline 
$t_2$ & 64 & 60.68 & 5.19 \\ \hline 
$t_3$ & 128 & 115.71 & 9.6 \\ \hline 
$t_4$ & 8 & 7.57 & 5.37 \\ \hline 
$t_5$ & 8 & 7.70 & 3.75 \\ \hline 
$t_6$ & 8 & 7.43 & 7.13 \\ \hline 
$t_7$ & 32 & 29.81 & 6.84 \\ \hline 
\textbf{AVG} & - & - & 6.2\\\hline
\end{tabular}

%%%%%%%%%%%%%%%%%% prevayler
\begin{tabular}{|c|r|r|r|} \hline
    test & \CodeIn{SPLat} & \tname{}  & Red(\%)\\ \hline
    \multicolumn{3}{c}{\textbf{Prevayler[All]}} \\ \hline
$t_1$ & 10 & 6.39 & 36.1 \\ \hline 
$t_2$ & 12 & 9.50 & 20.83 \\ \hline 
$t_3$ & 2 & 1.50 & 25.0 \\ \hline 
$t_4$ & 10 & 8.38 & 16.2 \\ \hline 
$t_5$ & 2 & 1.00 & 50.0 \\ \hline 
$t_6$ & 12 & 6.08 & 49.33 \\ \hline 
$t_7$ & 16 & 11.71 & 26.81 \\ \hline 
$t_8$ & 6 & 4.83 & 19.5 \\ \hline 
\textbf{AVG} & - & - & 30.47\\\hline
%\end{tabular}


%%%%%%%%%%%%%%%%%% jtopas
%\begin{tabular}{|c|r|r|} \hline
%    test & \CodeIn{SPLat} & \tname{} \\ \hline
    \multicolumn{3}{c}{\textbf{JTopas [All]}} \\ \hline
$t_{1}$ & 8 & 7.73 & 3.37 \\ \hline 
$t_{2}$ & 8 & 7.92 & 1.0 \\ \hline 
$t_{3}$ & 14 & 13.64 & 2.57 \\ \hline 
$t_{4}$ & 16 & 15.63 & 2.31 \\ \hline 
$t_{5}$ & 16 & 15.66 & 2.12 \\ \hline 
$t_{6}$ & 8 & 7.96 & 0.5 \\ \hline 
$t_{7}$ & 8 & 7.84 & 2.0 \\ \hline 
$t_{8}$ & 28 & 26.30 & 6.07 \\ \hline 
$t_{9}$ & 16 & 15.24 & 4.75 \\ \hline 
$t_{10}$ & 8 & 7.71 & 3.63 \\ \hline 
$t_{11}$ & 8 & 7.81 & 2.38 \\ \hline 
$t_{12}$ & 8 & 7.88 & 1.5 \\ \hline 
$t_{13}$ & 14 & 13.70 & 2.14 \\ \hline 
$t_{14}$ & 16 & 15.59 & 2.56 \\ \hline 
$t_{15}$ & 16 & 15.63 & 2.31 \\ \hline 
$t_{16}$ & 8 & 7.96 & 0.5 \\ \hline 
$t_{17}$ & 8 & 7.86 & 1.75 \\ \hline 
$t_{18}$ & 28 & 26.36 & 5.86 \\ \hline 
$t_{19}$ & 16 & 15.23 & 4.81 \\ \hline 
$t_{20}$ & 8 & 7.66 & 4.25 \\ \hline 
$t_{21}$ & 8 & 7.88 & 1.5 \\ \hline 
$t_{22}$ & 8 & 7.92 & 1.0 \\ \hline 
$t_{23}$ & 2 & 1.92 & 4.0 \\ \hline 
$t_{24}$ & 1 & 1.00 & 0.0 \\ \hline 
$t_{25}$ & 1 & 1.00 & 0.0 \\ \hline 
$t_{26}$ & 1 & 1.00 & 0.0 \\ \hline 
$t_{27}$ & 8 & 7.91 & 1.12 \\ \hline 
$t_{28}$ & 20 & 18.89 & 5.55 \\ \hline 
\textbf{AVG} & - & - & 2.48\\\hline

    \multicolumn{3}{c}{\textbf{Email[All]}} \\ \hline
$t_1$ & 1 & 1.00 & 0.0 \\ \hline 
$t_2$ & 30 & 17.98 & 40.07 \\ \hline 
$t_3$ & 40 & 26.62 & 33.45 \\ \hline 
$t_4$ & 40 & 28.73 & 28.18 \\ \hline 
$t_5$ & 40 & 26.62 & 33.45 \\ \hline 
$t_6$ & 40 & 28.44 & 28.9 \\ \hline 
$t_7$ & 40 & 28.44 & 28.9 \\ \hline 
$t_8$ & 40 & 27.91 & 30.23 \\ \hline 
$t_9$ & 40 & 26.28 & 34.3 \\ \hline 
$t_{10}$ & 40 & 28.25 & 29.38 \\ \hline 
$t_{11}$ & 40 & 29.29 & 26.78 \\ \hline 
$t_{12}$ & 40 & 27.47 & 31.33 \\ \hline 
$t_{13}$ & 40 & 28.16 & 29.6 \\ \hline 
$t_{14}$ & 40 & 26.45 & 33.88 \\ \hline 
$t_{15}$ & 30 & 20.89 & 30.37 \\ \hline 
\textbf{AVG} & - & - & 29.25\\\hline
\end{tabular}

%%%%%%%%%%%%%%%%%% elevator
\begin{tabular}{|c|r|r|r|} \hline
    test & \CodeIn{SPLat} & \tname{}  & Red(\%)\\ \hline
    \multicolumn{3}{c}{\textbf{Elevator [All]}} \\ \hline
$t_1$ & 1 & 1.00 & 0.0 \\ \hline 
$t_2$ & 10 & 8.29 & 17.1 \\ \hline 
$t_3$ & 10 & 8.47 & 15.3 \\ \hline 
\textbf{AVG} & - & - & 10.8\\\hline
%\end{tabular}

% %%%%%%%%%%%%%%%%% sudoku
%% \begin{tabular}{|c|r|r|} \hline
%%     test & \CodeIn{SPLat} & \tname{} \\ \hline
    \multicolumn{3}{c}{\textbf{Sudoku [All]}} \\ \hline
$t_1$ & 8 & 4.56 & 43.0 \\ \hline 
$t_2$ & 16 & 5.38 & 66.38 \\ \hline 
$t_3$ & 16 & 8.41 & 47.44 \\ \hline 
$t_4$ & 4 & 2.05 & 48.75 \\ \hline 
$t_5$ & 10 & 5.87 & 41.3 \\ \hline 
$t_6$ & 20 & 16.31 & 18.45 \\ \hline 
\textbf{AVG} & - & - & 44.22\\\hline
%\end{tabular}


%% %%%%%%%%%%%%%%%%%% zipme
%\begin{tabular}{|c|r|r|} \hline
%    test & \CodeIn{SPLat} & \tname{} \\ \hline
    \multicolumn{3}{c}{\textbf{ZipMe [All]}} \\ \hline
$t_1$ & 2 & 1.89 & 5.5 \\ \hline 
$t_2$ & 2 & 1.90 & 5.0 \\ \hline 
$t_3$ & 2 & 1.91 & 4.5 \\ \hline 
$t_4$ & 2 & 1.93 & 3.5 \\ \hline 
$t_5$ & 2 & 1.90 & 5.0 \\ \hline 
$t_6$ & 2 & 1.94 & 3.0 \\ \hline 
$t_7$ & 4 & 3.00 & 25.0 \\ \hline 
$t_8$ & 2 & 1.50 & 25.0 \\ \hline 
$t_9$ & 4 & 3.62 & 9.5 \\ \hline 
$t_{10}$ & 4 & 3.57 & 10.75 \\ \hline 
$t_{11}$ & 4 & 3.77 & 5.75 \\ \hline 
$t_{12}$ & 2 & 1.00 & 50.0 \\ \hline 
$t_{13}$ & 2 & 1.50 & 25.0 \\ \hline 
$t_{14}$ & 2 & 1.74 & 13.0 \\ \hline 
$t_{15}$ & 8 & 6.55 & 18.13 \\ \hline 
$t_{16}$ & 8 & 6.80 & 15.0 \\ \hline 
$t_{17}$ & 8 & 6.80 & 15.0 \\ \hline 
$t_{18}$ & 6 & 5.00 & 16.67 \\ \hline 
$t_{19}$ & 6 & 5.33 & 11.17 \\ \hline 
$t_{20}$ & 6 & 4.14 & 31.0 \\ \hline 
$t_{21}$ & 6 & 5.33 & 11.17 \\ \hline 
$t_{22}$ & 6 & 5.00 & 16.67 \\ \hline 
$t_{23}$ & 4 & 3.40 & 15.0 \\ \hline 
$t_{24}$ & 2 & 1.33 & 33.5 \\ \hline 
$t_{25}$ & 4 & 3.85 & 3.75 \\ \hline 
$t_{26}$ & 2 & 1.94 & 3.0 \\ \hline 
$t_{27}$ & 4 & 3.09 & 22.75 \\ \hline 
$t_{28}$ & 4 & 3.56 & 11.0 \\ \hline 
$t_{29}$ & 4 & 3.85 & 3.75 \\ \hline 
$t_{30}$ & 2 & 1.00 & 50.0 \\ \hline 
$t_{31}$ & 2 & 1.00 & 50.0 \\ \hline 
$t_{32}$ & 4 & 3.09 & 22.75 \\ \hline 
$t_{33}$ & 8 & 7.11 & 11.12 \\ \hline 
$t_{34}$ & 8 & 7.11 & 11.12 \\ \hline 
$t_{35}$ & 6 & 4.86 & 19.0 \\ \hline 
$t_{36}$ & 2 & 1.33 & 33.5 \\ \hline 
$t_{37}$ & 4 & 3.84 & 4.0 \\ \hline 
$t_{38}$ & 2 & 1.93 & 3.5 \\ \hline 
$t_{39}$ & 4 & 3.23 & 19.25 \\ \hline 
$t_{40}$ & 6 & 4.92 & 18.0 \\ \hline 
$t_{41}$ & 4 & 3.85 & 3.75 \\ \hline 
$t_{42}$ & 2 & 1.00 & 50.0 \\ \hline 
$t_{43}$ & 2 & 1.00 & 50.0 \\ \hline 
$t_{44}$ & 4 & 2.81 & 29.75 \\ \hline 
$t_{45}$ & 8 & 7.11 & 11.12 \\ \hline 
$t_{46}$ & 8 & 7.11 & 11.12 \\ \hline 
$t_{47}$ & 8 & 6.25 & 21.88 \\ \hline 
\textbf{AVG} & - & - & 17.83\\\hline
\end{tabular}

%\vspace{-5ex}
\end{tabular}

\caption{\label{fig:results-scenario-one}Red in number of configurations
explored for each test.  We show within brackets the upper bound on
the number of explored configurations we used in this experiment to
enable execution to finish in a reasonable amount of time.  For
example, the bound for Notepad was 100.}
%\vspace{-3.0ex}
\end{figure*}
\def\arraystretch{1}%


==> splat-gcc.tex <==
\textbf{\SPLKorat{} for GCC. } The initial version of \SPLKorat{} (used to evaluate SPLs) is not able to run GCC code, because: (1) it is coded in the same language of the subject programs used (Java). Consequently, it does not work for GCC, written in the C/C++ language; and (2) this version only considers boolean values (true/false or 0/1) for the configuration options, and \gcc{} has some options with multiple values.

In this context, it would be necessary developing another version of \SPLKorat{} to support both other languages (C/C++, for example) and multiple configuration option values. Therefore, we decided to build a more generic version of \SPLKorat{} (\CodeIn{SPLatFile}), by implementing a new instrumentation, and creating a map of  variables-to-option to deal with multiple values.

%In order to avoid developing another version of \SPLKorat{} in C language, we decided to monitor the feature variables (exercised during the test execution) using log files containing the values that feature variables assume during execution. This resulted in a new version of \SPLKorat{} (\CodeIn{SPLatFile}) for C/C++ and other languages, that supports those files and feature variables with multiple values. Both the \emph{instrumentation} and the \emph{variables-to-option map} were fundamental for \CodeIn{SPLatFile} structure.

Regarding Instrumentation, it is important to distinguish \emph{input option} from \emph{feature variable}. Input options correspond to the configuration parameters passed to the system, typically on the command line (\eg{}, ``\CodeIn{-O2}'') whereas feature variables are the program variables that reflect these options in code (\eg{}, ``\CodeIn{optimize}'').  To enable execution of \splat{} on \gcc{} (see Figure~\ref{fig:test_gcc}, line, we instrumented \gcc{} to monitor all accesses to feature variables by wrapping the uses of accessor macros with a call to a function we defined.  These macros are automatically generated from option definition files~\citep{gccoptionsdefs}.  The execution of each test on instrumented \gcc{} produces a log file containing the values that feature variables assume during execution.  

Regarding Variables-to-option map construction, to determine new input vectors from variable accesses we\Comment{ manually} constructed a map to express the correspondence between feature variables (with their values) and configuration options.\Comment{ This is necessary to determine new configuration inputs for test execution.}  It is important to note that the construction of this map can be automated (see~\citep{xu-etal-sosp2013}).  This map expresses, for example, the
correspondence of \CodeIn{optimize=2} with the option \CodeIn{-O2}.  From the log file of accessed variables produced
with the test run and the variable-option map\Comment{, from variables to values to options,}, \splat{} is able to generate new test inputs (\ie{}, option vectors).

